Generative Latent Alignment for Interpretable Radar Based Occupancy Detection in Ambient Assisted Living

In this work, we study how to make mmWave radar presence detection more interpretable for Ambient Assisted Living (AAL) settings, where camera-based sensing raises privacy concerns. We propose a Generative Latent Alignment (GLA) framework that combines a lightweight convolutional variational autoencoder with a frozen CLIP text encoder to learn a low-dimensional latent representation of radar Range-Angle (RA) heatmaps. The latent space is softly aligned with two semantic anchors corresponding to "empty room" and "person present", and Grad-CAM is applied in this aligned latent space to visualize which spatial regions support each presence decision. On our mmWave radar dataset, we qualitatively observe that the "person present" class produces compact Grad-CAM blobs that coincide with strong RA returns, whereas "empty room" samples yield diffuse or no evidence. We also conduct an ablation study using unrelated text prompts, which degrades both reconstruction and localization, suggesting that radar-specific anchors are important for meaningful explanations in this setting.

==> sec/method2.tex <==
\subsection{Semantic Radar VAE}

Our model takes as input 2D Range--Angle (RA) intensity maps computed from the raw
mmWave FMCW radar sweeps. We follow the standard processing chain: a Fast Fourier
Transform (FFT) along range and Doppler, followed by Capon/Minimum Variance
Distortionless Response (MVDR) beamforming for angle estimation \cite{abedi2024contactless}.
Each processed frame is stored as an image $x$ and resized to a fixed spatial
resolution $H \times W = 224 \times 224$. Although the underlying radar return
is single–channel, we store $x \in \mathbb{R}^{C \times H \times W}$ with
$C=3$ using a fixed colormap, mainly for logging and compatibility with
vision backbones.

Before training, we rescale the intensities of $x$ to $[0,1]$ and apply
instance-wise normalization. This step reduces global gain differences between
recordings and encourages the VAE to focus on the spatial RA pattern
(e.g., whether a compact reflection blob appears near a wall) rather than
absolute power \cite{abedi2024contactless}.

Given an input frame $x$, the encoder $E_{\phi}$ outputs the parameters of a
diagonal Gaussian posterior $q_{\phi}(z \mid x)$. In our implementation it
returns a mean vector $\mu = f_{\mu}(x)$ and a log–variance
$\log \sigma^2 = f_{\log \sigma^2}(x)$. The encoder consists of four strided
convolutional blocks that reduce the spatial resolution from $224 \rightarrow 14$,
followed by a flatten layer and two linear heads that produce $\mu$ and
$\log \sigma^2$ from the deepest feature maps. During training we draw
latent samples using the reparameterization trick \cite{kingma2019introduction},
\[
  z = \mu + \sigma \odot \epsilon, \quad \epsilon \sim \mathcal{N}(0, I),
\]
which allows gradients to flow through the stochastic sampling step and defines
the approximate posterior
\[
  q_{\phi}(z \mid x) = \mathcal{N}\big(z; \mu_\phi(x),
          \mathrm{diag}(\sigma^2_\phi(x))\big).
\]

The decoder $D_{\theta}$ mirrors the encoder with a stack of transposed
convolutions that upsamples $z$ back to the input resolution and produces a
reconstruction $\hat{x} = D_{\theta}(z)$. A final sigmoid activation ensures
$\hat{x} \in [0,1]$, so reconstructions can be compared directly with the
normalized input.

We train $E_{\phi}$ and $D_{\theta}$ with the standard VAE objective
\cite{kingma2013auto}: the evidence lower bound is written as
$L_{\mathrm{VAE}} = L_{\mathrm{recon}} + L_{\mathrm{KLD}}$.
Since RA frames are scaled to $[0,1]$, we use a per–pixel binary
cross-entropy reconstruction loss
\[
  L_{\mathrm{recon}} = \mathrm{BCE}(x,\hat{x})
  = -\sum_{u} \big[x_u \log \hat{x}_u + (1-x_u)\log(1-\hat{x}_u)\big],
\]
where $u$ indexes pixels and channels. The KL term penalizes deviation from an
isotropic Gaussian prior $p(z) = \mathcal{N}(0,I)$,
\[
  L_{\mathrm{KLD}} = D_{\mathrm{KL}}(q_{\phi}(z \mid x)\,\|\,p(z))
  = -\frac{1}{2} \sum_{j} \big(1 + \log \sigma_j^2 - \mu_j^2 - \sigma_j^2\big).
\]

Intuitively, $L_{\mathrm{recon}}$ keeps fine-grained RA structure
(e.g., the position and extent of reflection blobs), while
$L_{\mathrm{KLD}}$ regularizes the latent space so that nearby latent codes
interpolate smoothly between plausible RA patterns.

\subsection{Text-Anchor Latent Alignment with Frozen CLIP}

To relate latent codes to human concepts, we add a small alignment head on top
of the VAE mean $\mu$. The head encourages $\mu$ to sit close to text
embeddings produced by a frozen CLIP text encoder \cite{radford2021learning}.
We use two short prompts,
$T = \{t_0, t_1\}$, that describe an empty room and a person-present radar
heatmap. CLIP is treated purely as a fixed text feature extractor; any other
pretrained text encoder that provides a metric embedding space could be used in
its place.

The CLIP embedding dimension $D$ does not necessarily match the latent
dimension $d$, so we introduce a linear projection
$W \in \mathbb{R}^{D \times d}$ and map the latent mean to
$\tilde{\mu} = W \mu$. We then $\ell_2$–normalize both the projected latent and
the text anchors,
\[
  \bar{\mu} = \frac{\tilde{\mu}}{\|\tilde{\mu}\|_2}, \qquad
  \bar{t}_k = \frac{t_k}{\|t_k\|_2}.
\]

Cosine-similarity logits are computed as
$s_k = \tau\, \bar{\mu}^{\top}\bar{t}_k$, where $\tau$ is a scalar temperature
(initialized to $10.0$) that controls the sharpness of the alignment.
Let $y \in \{0,1\}$ denote the ground-truth class label. The alignment loss is
the cross-entropy between the logits $s=[s_0,s_1]$ and $y$,
\[
  L_{\mathrm{align}} = \mathrm{CE}(s,y).
\]

Samples labeled “person” are pulled towards the person anchor, while
“empty” samples are pulled towards the empty-room anchor. As a result, the
latent space develops an intrinsic semantic structure that we later probe with
Grad-CAM. Compared with radar-to-text generation pipelines that require extra
decoders and adversarial objectives \cite{otto2025talk}, this anchor-based
design keeps the architecture lightweight while still embedding radar domain
knowledge into the latent geometry.

\subsection{Latent-Space Explainability (Latent Grad-CAM)}

For explanations we adapt Grad-CAM \cite{selvaraju2019grad} to the third
convolutional block of the encoder. For a target class score $s_y$, we compute
gradients $\partial s_y / \partial F^c_{ij}$ with respect to the feature map
$F^c \in \mathbb{R}^{H \times W}$. Channel importance weights $\alpha_c$ are
obtained by global average pooling over spatial locations,
\[
  \alpha_c = \frac{1}{H W} \sum_i \sum_j
             \frac{\partial s_y}{\partial F^c_{ij}}.
\]

The latent Grad-CAM map is then formed as
\[
  L_{\mathrm{CAM}} = \mathrm{ReLU} \Big( \sum_c \alpha_c F^c \Big),
\]
which we upsample to the RA input resolution. To reduce noise, we average CAMs
over several small Gaussian perturbations of the input frame. The resulting
heatmap is smoother and highlights the RA regions that most strongly influence
the class score in the aligned latent space.


==> sec/result2.tex <==
\section{Experiments and Results}

We train the semantic radar VAE described in Section~\ref{sec:method} on a
binary presence dataset of RA maps with labels “empty room” and
“person present”. The objective combines reconstruction, alignment, and KL
regularization,
\[
  L = \lambda_r L_{\mathrm{recon}} +
      \lambda_a L_{\mathrm{align}} +
      \lambda_k L_{\mathrm{KLD}},
\]
with $\lambda_r = 5.0$, $\lambda_a = 1.0$, and $\lambda_k = 0.01$.
In practice, this choice keeps reconstruction as the dominant term while still
giving the text anchors enough weight to influence the latent geometry.
We optimize with Adam (learning rate $5\times 10^{-4}$), train for at most
$20$ epochs, and use early stopping with a patience of five epochs. The CLIP
text encoder is frozen throughout; gradients from $L_{\mathrm{align}}$ update
only the VAE parameters and the projection matrix $W$.

For the two anchors we use radar-specific prompts
\begin{align}
  t_0 &= f_{\text{text}}\big(
       \text{``radar heatmap of an empty room without any person''}\big),
  \\
  t_1 &= f_{\text{text}}\big(
       \text{``radar heatmap of a person present in the room''}\big),
\end{align}
where $f_{\text{text}}$ denotes the CLIP text encoder and
$t_k \in \mathbb{R}^D$ are the resulting text embeddings. Mentioning both
“radar heatmap” and the presence or absence of a person ties the anchors to the
sensing modality and to the binary label space we study.

Figures~\ref{fig:empty_cam} and~\ref{fig:person_cam} show qualitative examples
for one empty-room and one person-present RA frame. Each panel displays,
from left to right: (i) the input RA intensity map, (ii) the VAE reconstruction,
(iii) the latent Grad-CAM heatmap, (iv) the Grad-CAM overlay on the RA input,
and (v) a binary CAM mask obtained by thresholding the top $15\%$ of CAM values.

For the empty-room example (Figure~\ref{fig:empty_cam}), the RA input mainly
contains background clutter and horizontal bands caused by static multipath.
The reconstruction smooths small artefacts while preserving these bands. The
Grad-CAM map for the “empty room” anchor spreads its energy along the same
bands, and the overlay and mask pick out a small high-salience patch consistent
with reflections from furniture.

For the person-present example (Figure~\ref{fig:person_cam}), the RA input is
dominated by a single strong blob at a particular range–angle bin. The
reconstruction again reduces high-frequency noise but maintains the blob’s
position. The latent Grad-CAM map now concentrates on this region, producing a
sharply localized peak. Both the overlay and the binary mask focus on the blob
while suppressing most of the surrounding clutter. Together, these results
suggest that the aligned latent space can localize presence-related structure
in RA maps and that the Grad-CAM heatmaps are consistent with the way the VAE
represents the scene.

To probe the role of the text anchors, we perform a small prompt ablation. We
replace the radar-specific phrases above with unrelated natural-image prompts
such as “clouds in the sky” or “an iceberg floating in the ocean”. Under these
prompts the VAE still reconstructs plausible RA patterns, but for
person-present inputs the latent Grad-CAM becomes nearly uniform and the CAM
mask contains no clearly salient region. For empty-room inputs, the CAM is more
diffuse and no longer aligns with an intuitive RA structure. This behaviour
indicates that the semantics of the prompts matter: domain-appropriate radar
anchors are needed for the alignment head to produce localized, meaningful
evidence maps in our setting.

